Decoupled Spatial Temporal Graphs for Generic Visual Grounding

Visual grounding is a long-lasting problem in vision-language understanding due to its diversity and complexity. Current practices concentrate mostly on performing visual grounding in still images or well-trimmed video clips. This work, on the other hand, investigates into a more general setting, generic visual grounding, aiming to mine all the objects satisfying the given expression, which is more challenging yet practical in real-world scenarios. Importantly, grounding results are expected to accurately localize targets in both space and time. Whereas, it is tricky to make trade-offs between the appearance and motion features. In real scenarios, model tends to fail in distinguishing distractors with similar attributes. Motivated by these considerations, we propose a simple yet effective approach, named DSTG, which commits to 1) decomposing the spatial and temporal representations to collect all-sided cues for precise grounding; 2) enhancing the discriminativeness from distractors and the temporal consistency with a contrastive learning routing strategy. We further elaborate a new video dataset, GVG, that consists of challenging referring cases with far-ranging videos. Empirical experiments well demonstrate the superiority of DSTG over state-of-the-art on Charades-STA, ActivityNet-Caption and GVG datasets. Code and dataset will be made available.

==> tables/STG-UVG.tex <==

\begin{table*}[t]
\setlength{\tabcolsep}{2.6pt}
\caption{Comparisons of baseline methods and the proposed DSTG on the val and test sets of the new GVG benchmark. We also combines the SPG and TPG module with other methods to fulfill a thorough comparison.} %use I3D features. Methods with $\ddagger$ use I3D features extracted with SlowFast Network~\cite{feichtenhofer2019slowfast}.}
\centering
\begin{tabular}{ll cccc cccc}
    \toprule
    \multirow{2}{*} {} &\multirow{2}{*} {Method}& \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}} \textbf{Val set}\end{tabular}} &
    \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}} \textbf{Test set}\end{tabular}} \\ \cline{3-10}
    {}&{}& m\_vIoU & vIoU$_{@0.25}$ & vIoU$_{@0.5}$ & vIoU$_{@0.75}$
    & m\_vIoU & vIoU@$_{@0.25}$ & vIoU$_{@0.5}$ & vIoU$_{@0.75}$ \\ 
    \midrule
    \multirow{3}{*}{RoI-based} 
    & Random Anc.             & 8.7 & 16.8 & 11.3 & 7.5 
                                    & 8.2 & 15.5 & 10.7 & 7.1 \\ 
    {}& Mattnet~\cite{yu2018mattnet}/Sort   & 11.5 & 17.3 & 13.2 & 10.7 
                                    & 11.7 & 17.7 & 13.0 & 10.5 \\
    {}& STPR/Sort   & 12.1 & 17.8 & 14.6 & 11.4 
                 & 12.2 & 17.6 & 14.9 & 11.5 \\
    \midrule
    \multirow{3}{*}{Anchor-based}
    % & Mattnet  & 14.5 & 21.1 & 16.0 & 13.3 
    %                           & 14.3 & 20.8 & 15.5 & 13.4 \\
    {}& CTRL~\cite{gao2017tall}  & 16.4 & 23.3 & 18.1 & 14.7 
                               & 16.8 & 23.5 & 18.6 & 14.8 \\
    % {}& \textbf{SPG}                  & 18.3 & 24.8 & 19.8 & 16.2 
    %                           & 18.5 & 24.9 & 20.2 & 15.9 \\
    % \hline
    {}& TGN  & 17.7 & 24.2 & 19.3 & 16.3 
                               & 17.4 & 23.9 & 19.2 & 16.3 \\
    % {}& DGA                      & 20.6 & 26.7 & 22.4 & 18.2 
    %                           & 20.3 & 26.5 & 22.1 & 17.8 \\
    % {}& \textbf{SPG}                    & 21.0 & 27.5 & 23.3 & 19.8 
    %                           & 21.1 & 27.4 & 23.4 & 20.2 \\
    % \multirow{2}{*}{CBP~\cite{wang2020temporally}}& Mattnet  & 21.6 & 28.9 & 23.9 & 20.4 
    %                                  & 21.7 & 29.1 & 24.2 & 19.9 \\
    {}& CBP     & 22.9 & 30.3 & 25.3 & 21.4 & 23.1 & 30.6 & 25.4 & 21.6 \\
    % {}& \textbf{SPG}   & 24.2 & 31.5 & 26.5 & 22.7 & 23.8 & 31.1 & 25.8 & 22.0 \\
    \midrule
    \multirow{5}{*}{Graph-based}
    & DGA/CTRL  & 30.6 & 37.2 & 33.2 & 27.8 & 30.2 & 36.9 & 33.0 & 27.3 \\
    {} & WSSTG/CTRL  & 31.3 & 37.6 & 33.6 & 28.1 & 31.5 & 37.7 & 33.8 & 28.4 \\ %\cline{2-10}
    {} & DSTG w/o CL & 32.7 & 38.2 & 34.2 & 30.5 
       & 32.9 & 38.4 & 34.5 & 30.7 \\ 
    {} & DSTG w/o DB & 32.7 & 38.2 & 34.2 & 30.5 
       & 32.9 & 38.4 & 34.5 & 30.7 \\
    {} & \textbf{DSTG} & \textbf{32.7} & \textbf{38.2} & \textbf{34.2} & \textbf{30.5} 
       & \textbf{32.9} & \textbf{38.4} & \textbf{34.5} & \textbf{30.7} \\
    \bottomrule
\end{tabular}
% \vspace{1mm}
\label{tab:gvg_result}
% \vspace{-3mm}
\end{table*}


==> tables/TG-charades.tex <==
\setlength{\tabcolsep}{24pt}
\renewcommand{\arraystretch}{0.95}
\begin{table}[t]
\centering
\caption{We report mean average precision (mAP) computed following the same setting in ~\cite{sigurdsson2016hollywood} for temporal localization on Charades dataset.}
\scalebox{1}{
\begin{tabular}{l c}
\toprule
Method & mAP $\uparrow$ \\
\midrule
Predictive-corrective~\cite{dave2017predictive} & \phantom{0}8.9 \\
Two-stream + LSTM ~\cite{sigurdsson2016hollywood} & \phantom{0}9.6 \\
R-C3D ~\cite{xu2017r} & 12.7 \\
SSN ~\cite{zhao2017temporal} & 16.4 \\
I3D baseline ~\cite{piergiovanni2019temporal} & 17.2 \\
Super-events ~\cite{piergiovanni2018learning} & 19.4 \\
TGM ~\cite{piergiovanni2018learning} & 22.3 \\
Mavroudi\etal ~\cite{mavroudi2020representation} & 23.7 \\
Piergiovanni\etal ~\cite{piergiovanni2020avid} & 25.2\\

\midrule
\textbf{DeCLON (Ours)} & \textbf{28.3}\\
\bottomrule
\end{tabular}}
%\vspace{-1mm}
\label{tab:charades_sota}
\end{table}

